The Fundamental Parameters of Astrophysical Plasma Turbulence and its Dissipation: Nonrelativistic Limit

A specific set of dimensionless plasma and turbulence parameters is introduced to characterize the nature of turbulence and its dissipation in weakly collisional space and astrophysical plasmas. Key considerations are discussed for the development of predictive models of the turbulent plasma heating that characterize the partitioning of dissipated turbulent energy between the ion and electron species and between the perpendicular and parallel degrees of freedom for each species. Identifying the kinetic physical mechanisms that govern the damping of the turbulent fluctuations is a critical first step in constructing such turbulent heating models. A set of ten general plasma and turbulence parameters are defined, and reasonable approximations along with the exploitation of existing scaling theories for magnetohydrodynamic turbulence are used to reduce this general set of ten parameters to just three parameters in the isotropic temperature case. A critical step forward in this study is to identify the dependence of all of the proposed kinetic mechanisms for turbulent damping in terms of the same set of fundamental plasma and turbulence parameters. Analytical estimations of the scaling of each damping mechanism on these fundamental parameters are presented, and this information is synthesized to produce the first phase diagram for the turbulent damping mechanisms as a function of driving scale and ion plasma beta.

==> Makefile <==
#-=-=-=-=-=-=-=
#Script for packing and compiling
#Phase Diagram for Plasma Turbulence
#Started Aug 2019
#-=-=-=-=-=-=-= 
#Variables

PACK = Makefile \
	turbtheory23*.tex \
	figs/*ps jpp.* 
#	turbtheory23*.ps \
#	*.bib \
#	jpp.*

SH = 'which sh'
CSH = 'which csh'

#-=-=-=-=-=-=-=

#

all : paper  paper.ps

paper.bib: paper; bibtex turbtheory23; paper; paper

paper:
	latex turbtheory23; bibtex turbtheory23; latex turbtheory23

paper.ps:
	dvips -o turbtheory23.ps -t letter turbtheory23.dvi

paper.pdf:
	ps2pdf turbtheory23.ps

pack: 	
	tar -cvf turbtheory23_`date +'%y%m%d'`.tar ${PACK}; gzip turbtheory23_`date +'%y%m%d'`.tar

